Steering Feedback in Dynamic Driving Simulators: Road-Induced and Non-Road-Induced Harshness

Steering feedback plays a substantial role in the validity of driving simulators for the virtual development of modern vehicles. Established objective steering characteristics typically assess the feedback behavior in the frequency range of up to 30 Hz while factors such as steering wheel and vehicle body vibrations at higher frequencies are mainly approached as comfort issues. This work investigates the influence of steering wheel and vehicle body excitations in the frequency range between 30 and 100 Hz on the subjective evaluation of steering feedback in a dynamic driving simulator. A controlled subject study with 42 participants was performed to compare a reference vehicle with an electrical power steering system to four variants of its virtual representation on a dynamic driving simulator. The effects of road-induced excitations were investigated by comparing a semi-empirical and a physics-based tire model, while the influence of non-road-induced excitations was investigated by implementing engine and wheel orders. The simulator variants were evaluated in comparison to the reference vehicle during closed-loop driving on a country road in a single-blind within-subjects design. The subjective evaluation focused on the perception of road feedback compared to the reference vehicle. The statistical analysis of subjective results shows that there is a strong effect of non-road-induced steering and vehicle body excitations, while the effect of road-induced excitations is considerably less pronounced.

==> fig_Spider_RoadContactAllVars.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=2.5in]{fig_Spider_RoadContactVarAllVars39.pdf}
    \caption{Absolute value of Road contact ratings (higher is better)
    % TODO: Add legend
    }
    \label{fig_Spider_RoadContactAllVars}
    \end{figure}
    
